Dose-response modeling in high-throughput cancer drug screenings: An end-to-end approach

Personalized cancer treatments based on the molecular profile of a patient's tumor are an emerging and exciting class of treatments in oncology. As genomic tumor profiling is becoming more common, targeted treatments to specific molecular alterations are gaining traction. To discover new potential therapeutics that may apply to broad classes of tumors matching some molecular pattern, experimentalists and pharmacologists rely on high-throughput, in-vitro screens of many compounds against many different cell lines. We propose a hierarchical Bayesian model of how cancer cell lines respond to drugs in these experiments and develop a method for fitting the model to real-world high-throughput screening data. Through a case study, the model is shown to capture nontrivial associations between molecular features and drug response, such as requiring both wild type TP53 and overexpression of MDM2 to be sensitive to Nutlin-3(a). In quantitative benchmarks, the model outperforms a standard approach in biology, with ~20% lower predictive error on held out data. When combined with a conditional randomization testing procedure, the model discovers biomarkers of therapeutic response that recapitulate known biology and suggest new avenues for investigation. All code for the paper is publicly available at https://github.com/tansey/deep-dose-response.

==> app_all_batch_effects.tex <==
\section{Temporal batch effects for all stratifications}

Figures~\ref{fig:all_batch_effects} and~\ref{fig:all_control_prior_fits} show the temporal dependence and the time-evolved density fits, respectively, for all four stratifications.

\begin{figure}
\centering
\includegraphics[width=\textwidth]{figures/all-negative-controls-batches.pdf}
\caption{The median control well measurements after removing contaminated wells. The x-axis is the date ID of the experiment (exact dates are not given). Points were clustered into batches by simply thresholding on the days between experiments. All sites exhibit clear temporal batch effects.}
\label{fig:all_batch_effects}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\textwidth]{figures/all-control-prior-fits.pdf}
\caption{Negative control well medians over time, stratified by testing site and assay type. Despite being run on separate plates, there is clear temporal ``batch-effect'' bias. We leverage this dependence by fitting a time-evolving density estimate of the mean and variance, shown in orange.}
\label{fig:all_control_prior_fits}
\end{figure}






==> conclusion.tex <==
% !TEX root = main.tex
\section{Conclusion}
\label{sec:conclusion}
We have presented an alternative approach to predictive modeling of cancer drug response in high-throughput screening experiments. Through a case study on a public dataset of thousands of experiments, we demonstrated that such studies contain systematic biases in their controls. In addition to correcting for these biases, we outlined a generative modeling approach that captures inherent uncertainty in the data due to natural variation in cell growth. The generative approach was shown to outperform a typical biological analysis pipeline in a dosage imputation task. Further, we confirmed that all three major subsets of genomic information (mutations, copy number variants, and expression) contribute predictive power to the final model; this suggests that hospitals and researchers should expand their panels to include all possible information sets. We also demonstrated that a black box predictive model is capable of recapitulating known biology, including nonlinear genomic interactions incapable of being captured by a nonlinear model. The final model can be used by experimentalists to guide future experiments and accelerate the discovery process for novel targeted cancer therapeutics.

